CRANE: A Redundant, Multi-Degree-of-Freedom Computed Tomography Robot for Heightened Needle Dexterity within a Medical Imaging Bore

Computed Tomography (CT) image guidance enables accurate and safe minimally invasive treatment of diseases, including cancer and chronic pain, with needle-like tools via a percutaneous approach. The physician incrementally inserts and adjusts the needle with intermediate images due to the accuracy limitation of free-hand adjustment and patient physiological motion. Scanning frequency is limited to minimize ionizing radiation exposure for the patient and physician. Robots can provide high positional accuracy and compensate for physiological motion with fewer scans. To accomplish this, the robots must operate within the confined imaging bore while retaining sufficient dexterity to insert and manipulate the needle. This paper presents CRANE: CT Robotic Arm and Needle Emplacer, a CT-compatible robot with a design focused on system dexterity that enables physicians to manipulate and insert needles within the scanner bore as naturally as they would be able to by hand. We define abstract and measurable clinically motivated metrics for in-bore dexterity applicable to general-purpose intra-bore image-guided needle placement robots, develop an automatic robot planning and control method for intra-bore needle manipulation and device setup, and demonstrate the redundant linkage design provides dexterity across various human morphology and meets the clinical requirements for target accuracy during an in-situ evaluation.

==> misc/algorithm_backup.tex <==

% \begin{algorithm}[t!]
% \caption{IK}
% \label{alg:IK}

% \DontPrintSemicolon
% \SetKwInput{Param}{Parameters}
% \SetKw{break}{break}
%  \KwIn{$x_{target}$: target robot tip pose; $q_0$: initial joint configuration}
%  \Param{$q_{nominal}$: nominal joint configuration, $q_{high}$: upper joint limit; $q_{low}$: lower joint limit}
%  \KwOut{$\bf{q}$: updated joint configuration}


% \Repeat{$convergence \text{ then } \textbf{return } q$}
%  {
%     $e \gets \text{\sc calculatePoseError}(x_{target}, x_{current})$\par
%     %\lIf{$||e_{\text{pos}}||_2 < \epsilon_{pos} \text{ and } ||e_{\text{ori}}||_2 < \epsilon_{ori}$}{break}

%     $\Delta q_{pose} \gets K J^{\dagger} e $ \par
%     $\Delta q_{null} \gets K_{null}(I-J^T(JJ^T)^{\dagger}J)(q_{nominal}-q)$\par
%     $\Delta q \gets K_{\text{pos}}J_{\text{pos}}^{\dagger}e_{\text{pos}} + K_{\text{ori}}J_{\text{ori}}^{\dagger} e_{\text{ori}}$  \par
%     $\text{\sc clip}(q + \Delta q_{pose} + \Delta q_{null}, q_{low}, q_{high})$
%     % $\Delta q \gets \text{\sc IK Step}(x_{target}, \bf{J}) $ \par
%     % $q \gets \text{\sc clip}(q + \Delta q, q_{low}, q_{high})$ \par
%  }

% \end{algorithm}


% \begin{algorithm}[t!]
% \caption{Controller Step}
% \label{alg:Controller_step}

% \DontPrintSemicolon
% \SetKwInput{Param}{Parameters}
% \SetKw{break}{break}
%  \KwIn{$x_{target}$: target robot tip pose; {$x_{current}$: current robot tip pose; $\bf{q}$: current joint configuration}}
%  \Param{$q_{nominal}$: nominal joint configuration, $q_{high}$: upper joint limit; $q_{low}$: lower joint limit}
%  \KwOut{target joint configuration}

% $e \gets \text{\sc calculatePoseError}(x_{target}, x_{current})$\par
% $\Delta q_{pose} \gets K J^{\dagger} e $ \par
% $\Delta q_{null} \gets K_{null}(I-J^T(JJ^T)^{\dagger}J)(q_{nominal}-q)$\par

% \textbf{return} {$\text{\sc clip}(q + \Delta q_{pose} + \Delta q_{null}, q_{low}, q_{high})$}

% \end{algorithm}



% \begin{algorithm}[bth!]
% \caption{Global Planner}\label{alg:global}
% \begin{algorithmic}

% \Procedure{Planner}{$x_{target}, q_0; q_{high}, q_{low}; c(\cdot), IK(\cdot)$}

% \EndProcedure

% \Procedure{minimize}{$q_0; c(\cdot), IK(\cdot)$}
%     \State $q \gets q_0$
%     \State $q[5 \colon 6] \gets q_{redundant}$ \Comment{Opt. variable} \\
%     \State $q \gets IK(x_{target, q)}$
%     \State $c_{adjustable} \gets 0$
%     \For{$x_{temp} \in x_{dexterous}$}
%         \State $q_local \gets LOCAL\_CONTROLLER(x_{temp}$
%         \If{q_local \not \in q_{free}}
%             \State{ $c_{adjustable} \gets 10 $
%         \EndIf
%     \EndFor
%     \State $c \gets c_{dexterity}(q) + c_{adjustable}$ \Comment{Cost function} \\
% \EndProcedure

% \Procedure{ik}{$x_{target}, q_0; q_{high}, q_{low}, \epsilon_{pos}, \epsilon_{ori}; fk(\cdot)$}
% \State $q \gets q_0$
% \For{$i=0;i<50;i++$}
%         \State $q[5 \colon 6] \gets q_0[5 \colon 6]$
%         \State $e_{\text{pos}} \gets x_{\text{target}} - fk(q)$
%         \State $e_{\text{ori}} \gets \angle(z_{\text{targ}} z_{\text{meas}}) (z_{\text{targ}} \times z_{\text{meas}}) $
%         \If{$||e_{\text{pos}}||_2 < \epsilon_{pos} \text{and} ||e_{\text{ori}}||_2 < \epsilon_{ori}$}
%             \State return $q$
%         \EndIf
%         \State $\Delta q \gets K_{\text{pos}}J_{\text{pos}}^{\dagger}e_{\text{pos}} + K_{\text{ori}}J_{\text{ori}}^{\dagger} e_{\text{ori}} $
%         \State $q \gets \text{clip}(q + \Delta q, q_{low}, q_{high})$
%         \EndIf
% \EndFor \\

% \Return -1
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[t!]
% \caption{Dexterous Configuration Generator}
% \label{alg:global_planner}

% \DontPrintSemicolon
% \SetKwInput{Param}{Parameters}
% \SetKw{break}{break}
%  \KwIn{$x_{target}$: target robot tip pose, $q_0$: initial joint configuration}
%  \Param{$q_{high}$: upper joint limit; $q_{low}$: lower joint limit; $c({q})$: cost function for a configuration}
%  \KwOut{$\bf{q^*}$: optimal robot joint configuration}

% \tcp{Initialize $q$ via IK with full Jacobian}

% %$q_0 \gets \text{\sc sampleFrom}\mathcal{U}(q_{low}, q_{high})$ \par
% %$q_{0} \gets \text{\sc IK} (x_{target}; \; q_0; J )$ \par
% \While{$not \; converged$}%\text{ then } \textbf{return } q$}
%  {
%     $e \gets \text{\sc calculatePoseError}(x_{target}, \text{\sc FK}(q_0))$\par
%     %\lIf{$||e_{\text{pos}}||_2 < \epsilon_{pos} \text{ and } ||e_{\text{ori}}||_2 < \epsilon_{ori}$}{break}
%     %$U \gets $ \par
%     $q_0 \gets q_0 + K J^{\star}e$% + (I-J^{\star}J)U$ \par
%     %$\Delta q_{null} \gets K_{null}(I-J^T(JJ^T)^{\dagger}J)(q_{nominal}-q)$\par
%     %$\Delta q \gets K_{\text{pos}}J_{\text{pos}}^{\dagger}e_{\text{pos}} + K_{\text{ori}}J_{\text{ori}}^{\dagger} e_{\text{ori}}$  \par
%     %$\text{\sc clip}(q + \Delta q_{pose} + \Delta q_{null}, q_{low}, q_{high})$
%     % $\Delta q \gets \text{\sc IK Step}(x_{target}, \bf{J}) $ \par
%     % $q \gets \text{\sc clip}(q + \Delta q, q_{low}, q_{high})$ \par
%  }


% \tcp{Optimize for $q^*$ via redundant joints}
% %$c \gets \infty$\par
% \While{$\text{not minimized}(c) \text{ then } \textbf{return } q^*$}
% {
%     %$q \gets q_0$\par
%     %\tcp{Optimizer samples a configuration for the redundant joints}
%     $q \gets \text{\sc sampleRedundantConfig}(q_0)$ \par
%     % \Repeat{$convergence \text{ then } \textbf{return } q$}
%     % {
%     % $q_{redundant} \gets \hat q_{redundant}$\par
%     % $e_{\text{pos}} \gets x_{\text{target}} - fk(q_0)$\par
%     % $e_{\text{ori}} \gets \angle(z_{\text{targ}}\par z_{\text{meas}}) (z_{\text{targ}} \times z_{\text{meas}})$\par
%     % \lIf{$||e_{\text{pos}}||_2 < \epsilon_{pos}             \text{and} ||e_{\text{ori}}||_2 < \epsilon_{ori}$}{break}
%     % $\Delta q \gets K_{\text{pos}}J_{\text{pos}}^{\dagger}e_{\text{pos}} + K_{\text{ori}}J_{\text{ori}}^{\dagger} e_{\text{ori}}$  \par
%     % $q \gets \text{\sc clip}(q + \Delta q, q_{low}, q_{high})$ \par
%     % }

%     %\tcp{Push robot back to target pose using non-redundnat joints and augmented jacobian}
%     %$q \gets \text{\sc IK} (x_{target}; \; q_0; J_{redundant})$ \par
%     \While{$not \; converged$}%\text{ then } \textbf{return } q$}
%          {
%             $e \gets \text{\sc calculatePoseError}(x_{target}, \text{\sc FK}(q))$\par
%             $q \gets q + K J_{aug}^{\star} e$ \par % + (I-J^{\dagger}J)U$ \par
%          }
%     %\tcp{Evaluate dexterity and cost for this robot configuration}
%     $c_{adjustable} \gets 0$ \par
%     \ForEach{$x_{local} \in x_{dexterous}$}
%     {
%     %\tcp{IK with nullspace constraint}
%      %   \tcp{IK with full jacobian and nullspace controller to stay near nominal configuration}
%         $q_{local} \gets q$ \par
%         \While{$not \; converged$}%\text{ then } \textbf{return } q$}
%          {
%             $e \gets \text{\sc calculatePoseError} (x_{local}, \text{\sc FK}(q_{local}))$\par
%             $q \gets q + K J_{aug}^{\star} e + (I-J_{aug}^{\star}J_{aug})( q-q_{local} ) $ \par
%             \lIf{$q_{local} \not \in q_{free}$}{$c_{adjustable} \gets C_{infeasible} $}
%          }
%         %$q_{local} \gets \text{\sc IK}(x_{local}; q; J; q; K_{null})$ \par
%     }
%     $c \gets c_{dexterity}(q) + c_{adjustable}$ \par
% }
% %$\bf{q} \gets RRT(q_0, q_{n}^*$ \par
% \textbf{return} {$\bf{q}^*$}
% \end{algorithm}
 

==> text/table_dh_parameters.tex <==

% The DH parameters define the position of the next frame relative to the previous frame as $\bm{c}_{n+1} =  \bm{c}_{n}+ a \bm{x}_{n}+ D z_{n+1}$ and orientation relative to the previous frame.
% % \begin{equation}
% %     c_{n+1} = c_n + a x_n + d z_{n+1}
% % \end{equation}
% % and orientation relative to the previous frame
% % \begin{equation}
% %     R_{n+1} = 
% %     \setlength{\arraycolsep}{3pt}
% %     \renewcommand{\arraystretch}{0.8}
% % R_n \begin{bmatrix}
% % %\centering
% % 1  & 0  & 0 \\
% % 0  & \cos \alpha  & -\sin\alpha \\
% % 0 & \sin \alpha & \cos \alpha  \\
% % \end{bmatrix}
% % \begin{bmatrix}
% % %\centering
% % \cos \theta   & -\sin \theta  & 0 \\
% % \sin \theta   & \cos \theta  & 0\\
% % 0 & 0 & 1  \\
% % \end{bmatrix}
% % \end{equation}
% where $ R_{n}$ is the orientation and $ c_{n}$ is the position of the $ n$th frame relative to the robot's base frame, $ B$, and $ q_{n}$ is the position of the $ n$th joint. 
